Deep Point Set Resampling via Gradient Fields

3D point clouds acquired by scanning real-world objects or scenes have found a wide range of applications including immersive telepresence, autonomous driving, surveillance, etc. They are often perturbed by noise or suffer from low density, which obstructs downstream tasks such as surface reconstruction and understanding. In this paper, we propose a novel paradigm of point set resampling for restoration, which learns continuous gradient fields of point clouds that converge points towards the underlying surface. In particular, we represent a point cloud via its gradient field -- the gradient of the log-probability density function, and enforce the gradient field to be continuous, thus guaranteeing the continuity of the model for solvable optimization. Based on the continuous gradient fields estimated via a proposed neural network, resampling a point cloud amounts to performing gradient-based Markov Chain Monte Carlo (MCMC) on the input noisy or sparse point cloud. Further, we propose to introduce regularization into the gradient-based MCMC during point cloud restoration, which essentially refines the intermediate resampled point cloud iteratively and accommodates various priors in the resampling process. Extensive experimental results demonstrate that the proposed point set resampling achieves the state-of-the-art performance in representative restoration tasks including point cloud denoising and upsampling.

==> components/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> sections/50-application.tex <==
\section{Applications to Point Cloud Restoration}
In this section, we introduce representative applications of the proposed point set resampling method, including point cloud denoising and point cloud upsampling. 

\subsection{Point Cloud Denoising}
\label{subsec:exp_denoising}
\red{WH: add a figure here.}

Point clouds are often perturbed by noise, which comes from hardware, software or environmental causes. 
Hardware wise, noise occurs due to the inherent limitations
of the acquisition equipment. Software wise, in the case of generating point clouds with existing algorithms, points may locate somewhere completely wrong due to imprecise triangulation (\eg, a false epipolar matching). Environmentally, outliers
may appear due to the surrounding contamination, such as dust in the air. Noise corruption directly affects the subsequent applications of point clouds.

Assuming an additive noise model for a point cloud, namely, 

As we described in Eq~\ref{eq:denoise}, it is straightforward to use the proposed method to perform denoising task. The noisy point cloud in this task serves as the context point cloud and the initial query point cloud. What must be acknowledged is that it's hard to model the density function from the noisy point cloud, but we don't need a accurate result hence we can expect the neural network to accomplish the task. Then, we can use the resample algorithm to guide the noisy points move to the underlying surface gradually.




\subsection{Point Cloud Upsampling}
\label{sec:ups}
%\red{WH: add a figure here.}

Give a point cloud containing $N$ points, our goal is to infer more points and to generate a dense point cloud consisting of $rN$ points.To apply the proposed method, we first need to roughly upsample it into a denser point cloud. Here we have two different approaches. The first one is to simply perturb the sparse point cloud by slight Gaussian noise independently for $r$ times, leading to a denser but noisy point cloud with $rN$ points. The second method is adopting a light-weighted neural network as coarse generator, referring to the idea of Dis-PU \cite{li2021point}. We will introduction the implementation of the network in detain in Chapter~\ref{sec:experiment:upsampling} 

The goal of aforementioned two methods is to obtain a denser point cloud. The dense point cloud is likely to be noisy and non-uniform, however these problems will be solved in following procedure. The original point cloud which is relatively sparse however clean contains the information of the supporting manifold, hence it can acts as the context point cloud. Subsequently, the generated dense point cloud is fed into the network. Our model learns the vector field of the dense point cloud and update the coordinates of the points iteratively according to Eq.~\ref{eq:denoise}, finally leading to the real target point cloud. We will present the experimental results in detail in Chapter \ref{sec:experiments}.





% \subsection{Point Cloud Reconstruction}
% \red{Consider to remove as it is for visualization.}
% After using our method to get denoised or high-resolution point clouds, we reconstruct 3D surfaces from point samples in this section. Here we mainly use Poisson Surface Reconstruction\cite{kazhdan2006poisson}, which is based on marching cubes algorithm. The key insight is that .




%\section{Analysis}
%\label{sec:analysis}
%In this section, We will analyse our method in detail, including its unique properties and advantages and how it unifies point cloud denoising and upsampling


 
%Such property blablabla....
%regularization  GTV GLR -> 
%repulsion loss ( PUNET ) -> get_loss_vec 



%\subsection{From Denoising to Upsampling}
%In this section, we will elaborate on how our method which derives from denoising can be applied on upsampling. In denoising task, it is nature to learn the vector field which points to the underlying surface of the object. By performing the iterative optimizing methods which is similar to gradient ascent, the noisy point cloud can finally converge to the corresponding clean one. As for upsampling, given a sparse point cloud with $N$ points as input, we first need to roughly upsample it into a point cloud containing $rN$ points. We will describe our rough upsample method in Section~\ref{sec:experiment:upsampling}. Subsequently, we can use our method to learn the vector field of the dense point cloud which leads to the real target point cloud.

%With this simple technique, our model can unify upsampling and denoising as a fundamental point set resampling problem. That is, we upsample the sparse input to a denser one with noise, and resample it according to the learned vector field.  




==> tables/ablation.tex <==
\begin{tabular}{l|ccccccccccccccc}
\toprule
Dataset: PU & \multicolumn{2}{c}{10K, 1\%} & \multicolumn{2}{c}{10K, 2\%} & \multicolumn{2}{c}{10K, 3\%} & \multicolumn{2}{c}{10K, 4\%} & \multicolumn{2}{c}{10K, 5\%} &
\multicolumn{2}{c}{10K, 7\%} &
\multicolumn{2}{c}{10K, 10\%} &\\
Ablation & CD & P2M & CD & P2M & CD & P2M & CD & P2M & CD & P2M & CD & CD\\
\midrule
% \bf Rep  & 2.463 & 0.381 & 3.278 & 0.881 & 4.098 & 1.514 & & \\
% \bf GTV & 2.413 & 0.392 & 3.365 & 0.846 & 4.155 & 1.436 & &\\
\bf GLR & 2.426 & 0.375 & 3.294 &  & \bf{3.910} & \bf{1.150} & 4.746 & & 5.695& &8.285 & 13.364\\
\bf RGLR & 2.382 & 0.324 & 3.282 &  & 3.892 & &  & & 5.605& &8.100 & 13.153\\
\bf Original & 2.353 & 0.306 & 3.350 & 0.734 & 4.075 & 1.242 & 4.832 & & 5.820 & & 8.642 & 14.172\\
\bottomrule
\end{tabular}


==> tables/blensor.tex <==
\begin{tabular}{c|cc|cccc|c}
\toprule
 & MRPCA & GLR & PCNet & GPDNet & DMR & DenoiseGF & Ours \\
\midrule
CD & 
 2.886 & 2.663 & 3.137 & 5.909 & 2.764 &  2.616 & \textbf{2.552}\\
P2M & 
 1.933 & 1.920 & 2.142 & 4.557 & 1.910 &  1.847 & \textbf{1.783} \\
\bottomrule
\end{tabular}
